On Partial Opimality by Auxiliary Submodular Problems

In this work, we prove several relations between three different energy minimization techniques. A recently proposed methods for determining a provably optimal partial assignment of variables by Ivan Kovtun (IK), the linear programming relaxation approach (LP) and the popular expansion move algorithm by Yuri Boykov. We propose a novel sufficient condition of optimal partial assignment, which is based on LP relaxation and called LP-autarky. We show that methods of Kovtun, which build auxiliary submodular problems, fulfill this sufficient condition. The following link is thus established: LP relaxation cannot be tightened by IK. For non-submodular problems this is a non-trivial result. In the case of two labels, LP relaxation provides optimal partial assignment, known as persistency, which, as we show, dominates IK. Relating IK with expansion move, we show that the set of fixed points of expansion move with any "truncation" rule for the initial problem and the problem restricted by one-vs-all method of IK would coincide -- i.e. expansion move cannot be improved by this method. In the case of two labels, expansion move with a particular truncation rule coincide with one-vs-all method.

==> tex/autarkies.tex <==
%\section{Autarkies}
%Let us clarify several questions about autarkies on their own: given a pair $(x^{\rm min}, x^{\rm max})$, is it difficult to verify the autarky property? Does there exist an autarky, which would provide the most amount of domain constraints? The following example shoes that verifying autarky property is at least as difficult as solving minimization problem~\eqref{energy minimization}.
%\begin{example} Consider energy minimization with two or more labels. Let $f^* = \min_{x\in \L} \f(x)$. It is, in general, an NP-hard problem to compute. Let us construct energy $\f'$ with all pairwise and singleton terms replicating $\f$, but with one extra label, $L+1$, for each variable. Pairwise terms linking to this label are set to infinity: $f'_{st}(L+1,i) = f'_{st}(i,L+1)=\infty$. Let $C$ be some constant and set singleton terms $f'_s(L+1) = C/|\V|$. Then $(L+1,L+1)$ is a strong autarky for $\f'$ iff $C < f^*$. If we had an algorithm to verify autarky property, we would be able to answer the question $C < f^*$ for any given $C$, and determine $b$ bits of $f^*$ using $b$ such questions. This would suffice to compute $f^*$ for problems with integer terms.
%\end{example}
%\todo{verify with BoroshHammer}
%%
%\mypar{Semilattice of Autarkies}
%%In this section we study the question, whether there exist an autarky which provides the most amount of domain constraints.
%\begin{definition}A {\em join} of two autarkies $(x^1,x^2)$, $(y^1,y^2)$ is 
%the autarky $(x^1 \vee y^1, x^2 \wedge y^2)$.
%\end{definition}
%%Let us show that the join is indeed an autarky. 
%The join of two strong autarkies is always a strong autarky, but for weak autarkies additional condition have to be satisfied in order that their join would be an autarky.
%%The join of a strong autarky and a weak autarky is a 
%\begin{proof}
%From definition of autarkies, we have
%\begin{equation}\label{join:l1}
%%\begin{split}
%\f( (((x \vee x^1)\wedge x^2) \vee y^1) \wedge y^2 ) \leq \f((x \vee x^1)\wedge x^2) \leq \f(x)
%\end{equation}
%%Let us verify that
%Note, that for $x^1 \leq x^2$ we have $(x \vee \x^1) \wedge x^2 = (x \wedge \x^2) \vee x^1$.
%We can rewrite the labeling in RHS as follows
%\begin{equation}
%\begin{split}
%((x \vee x^1)\wedge x^2) \vee y^1) \wedge y^2 = \\
%((x \wedge x^2) \vee  (x^1 \vee y^1) ) \wedge y^2 \doteq\\
%(x \wedge (x^2 \wedge y^2) ) \vee  (x^1 \vee y^1),
%\end{split}
%\end{equation}
%where doted equality holds if $y^2\geq x^1$. This is satisfied for strong autarkies, because it would be a contradiction that all optimal labellings are below $y^2$ and above $x^1$. For weak autarkies there may exist some optimal labellings which are below $y^2$ and some optimal labellings which are above $x^1$ but with empty intersection, so that there is no optimal labellings which are both below $y^2$ and above $x^1$.
%\par
%It can be verified that the join of two strong autarkies is strong. The join of a strong autarky with a weak autarky is also always an autarky (weak).
%\end{proof}
%We now can claim the {\em most powerful} strong autarky to be the join of all strong autarkies. %The following example shows that computing it for a multi-label problem is NP-hard.

